Multi-Agent Motion Planning with B\'ezier Curve Optimization under Kinodynamic Constraints

Multi-Agent Motion Planning (MAMP) is a problem that seeks collision-free dynamically-feasible trajectories for multiple moving agents in a known environment while minimizing their travel time. MAMP is closely related to the well-studied Multi-Agent Path-Finding (MAPF) problem. Recently, MAPF methods have achieved great success in finding collision-free paths for a substantial number of agents. However, those methods often overlook the kinodynamic constraints of the agents, assuming instantaneous movement, which limits their practicality and realism. In this paper, we present a three-level MAPF-based planner called PSB to address the challenges posed by MAMP. PSB fully considers the kinodynamic capability of the agents and produces solutions with smooth speed profiles that can be directly executed by the controller. Empirically, we evaluate PSB within the domains of traffic intersection coordination for autonomous vehicles and obstacle-rich grid map navigation for mobile robots. PSB shows up to 49.79% improvements in solution cost compared to existing methods.

==> backup_related.tex <==

    {\color{blue} 
    bullet points: 
    1. Explain why use centralized method but decentralized method
    1.1. discuss common method in exploration
    1.2. discuss related work in multi-agent exploration with unknown initial pose
    2. Discuss method used in Map merge (mainly on unknown initial pose)
    }
    \textbf{Multi-agent exploration strategy.} Multi-agent exploration has been studied by researchers for over decades from multiple angles. 
    Current methods on map merge can be divided into centralized and decentralized, in this problem, we will use map merge module to get relative position which requires relative high computation cost. Thus, this paper use a centralized framework for exploration. We will focus on centralized multi-agent exploration methods.
    One of the most common methods in the formulation of exploration is using frontiers, which represents the area between explored space and unknown space \cite{yamauchi1997frontier, holz2010evaluating, dornhege2013frontier, cieslewski2017rapid, batinovic2021multi, orvsulic2019efficient}. 
    Based on the frontiers in the exploring map, the multi-agent exploration algorithm coordinate the robots by minimizing the overall cost and utility for each agent to cover all the frontiers \cite{cieslewski2017rapid, renzaglia2019combining, faria2019applying}. 
    Using information theory is another popular approach for solving the exploration problem \cite{bourgault2002information, stachniss2005information, carrillo2018autonomous}. In those works, the space of the exploring environment is usually divided into grids or voxels. Then, based on the exploring status of the cell, the potential information gained for future actions is estimated. 
    The follow-up multi-agent exploration algorithm chooses the actions of each agent which can maximize the total information gain across all agents \cite{burgard2005coordinated, nieto2014coordination}. However, most of the above-mentioned works are based on greedy strategies which are hard to get the global optimized result. 
    Recently, Rapidly-exploring Random Tree (RRT) \cite{lavalle1998rapidly, bircher2016receding, witting2018history} and Rapidly-exploring Random Graph(RRG) \cite{karaman2011sampling} based methods get extended to solve exploration problems. In \cite{bircher2016receding}, a heuristic exploration strategy, which is based on RRT, was proposed. This method view the node of RRT as viewpoints and select the next viewpoint that can maximize the reward function. In \cite{dang2019graph}, Dang et al. proposed a exploration architecture which combines local-planner and global-planner architecture. The local planner uses a rapidly-exploring random graph for local subspace path planning and collision avoidance. The global planner is used when the re-position of robot is needed.
    Recently, Chao et al. \cite{cao2021tare} proposed a hierarchical framework for single-agent exploration in a complex 3-D environment. The method maintains a coarse global map and a detailed local subspace map simultaneously. Then, it optimizes an overall exploration path and produces a kinodynamically feasible local path.
    Apart from the above methods, topological based \cite{choset2000sensor, acar2002sensor} and reinforcement learning based methods also attracted a lot of interest \cite{wang2019influence}.
    % The current multi-agent exploration research strongly depends on each agent's relative position or frequent changes in their relative position. Few works are done on the exploration of large-scale 3D environment utilizing multi-robot systems, which do not have any access to their relative pose.

   
    \begin{figure*}[!t]
        \centering
        \includegraphics[width=\linewidth]{Imgs/sec3/framework.pdf}
        \caption{\textbf{The overall framework of MrExplorer.}
        The overall structure comprises two components: the active map merge and sub-map multi-agent exploration.
        In the active map merge, the inner connections of the agents are increased by actively exploring the overlap region. The merged sub-map is provided along with the relative pose of agents on the sub-map.
        Given the sub-map, the multi-agent explorer will use a hierarchical planner for the exploration path planning of each agent.}
        \label{fig:OverallFramework}
    \end{figure*}
    
    
    \textbf{Large scale map merging and data association} 3D map merging problem can be defined as integrating different sub-maps with or without initial estimation, where the sub-maps model the 3D space which is usually represented into 3D point clouds, occupancy grids \cite{carpin2008fast, hornung2013octomap}, or 3D meshes \cite{rosinol2021kimera}. Map merging problem can be solved with initial estimation \cite{carpin2008fast, tian2022kimera, rosinol2021kimera, rusinkiewicz2001efficient} or without relative pose.
    Mathieu et al. proposed a visual appearance‐based multi-session mapping system without needing an initial pose estimation. This method uses an appearance‐based loop closure detection approach with the memory management to deal with large‐scale and long‐term online operations \cite{labbe2019rtab}. Renaud et al. proposed a street block-like global map merging framework which uses distinguishable semantic objects for data association \cite{dube2020segmap, yin2022automerge}. 
    The above-mentioned methods mainly rely on data association to get the interconnections between sub-maps by encoding them into descriptors and conducting global matching. Traditionally, common methods for descriptor extraction encode the raw input scan and image into bag-of-words vectors \cite{galvez2012bags} or learned full-image descriptors \cite{arandjelovic2013all}.
    To alleviate the insufficiency under illumination or seasonal changes for single input feature extraction, sequence-based place recognition methods were introduced to avoid mismatching. In \cite{milford2012seqslam, yin2020seqspherevlad}, a sequence-based place recognition method was proposed which uses the difference of a sequence of observations to provide light-invariant place recognition ability. In {\color{red} we'll cite automerge here}, the RANSAC-based data association method was provided to remove the outlier in the sequence matching.
    However, the success of the data association is still highly reliant on the overlap distance and overlap features. In large scale environment, it is hard to guarantee enough distance of overlap. 
    Only a few works were done to merge the global map actively. 
    In \cite{caccavale2019trust}, an active exploration strategy was proposed which actively verified if the sub-maps are correctly associated. But this method was limited to 2D environments and didn't apply to large-scale environments. 
